Graph Spatio-Spectral Total Variation Model for Hyperspectral Image Denoising

The spatio-spectral total variation (SSTV) model has been widely used as an effective regularization of hyperspectral images (HSI) for various applications such as mixed noise removal. However, since SSTV computes local spatial differences uniformly, it is difficult to remove noise while preserving complex spatial structures with fine edges and textures, especially in situations of high noise intensity. To solve this problem, we propose a new TV-type regularization called Graph-SSTV (GSSTV), which generates a graph explicitly reflecting the spatial structure of the target HSI from noisy HSIs and incorporates a weighted spatial difference operator designed based on this graph. Furthermore, we formulate the mixed noise removal problem as a convex optimization problem involving GSSTV and develop an efficient algorithm based on the primal-dual splitting method to solve this problem. Finally, we demonstrate the effectiveness of GSSTV compared with existing HSI regularization models through experiments on mixed noise removal. The source code will be available at https://www.mdi.c.titech.ac.jp/publications/gsstv.

==> tab_running_efficiency.tex <==
\begin{table*}[t]
	\begin{center}
		\caption{The actual running times per iteration [s] for Beltsville denoising.}
		\label{tab:running_efficiency}
% 		\scalebox{0.90}{
		\begin{tabular}{c ccccccc}
		    \toprule
	            & HTV & SSTV & TDL & ITSReg & LRTDTV & GSSTV & LRTDTV+GSSTV \\
            \cmidrule(lr){1-8}
		        time [s] & 0.0097 & 0.0091 & 0.1081 & 60.0326 & 0.1380 & 0.0093 & 3.0086\\
		        
			\bottomrule
		\end{tabular}
% 		}
\end{center}
\end{table*}
